On the natural domain of Bregman operators

The Bregman proximal mapping and Bregman-Moreau envelope are traditionally studied for functions defined on the entire space $\mathbb{R}^n$, even though these constructions depend only on the values of the function within (the interior of) the domain of the distance-generating function (dgf). While this convention is largely harmless in the convex setting, it leads to substantial limitations in the nonconvex case, as it fails to embrace important classes of functions such as relatively weakly convex ones. In this work, we revisit foundational aspects of Bregman analysis by adopting a domain-aware perspective: we define functions on the natural domain induced by the dgf and impose properties only relative to this set. This framework not only generalizes existing results but also rectifies and simplifies their statements and proofs. Several examples illustrate both the necessity of our assumptions and the advantages of this refined approach.

==> TeX/Preamble.tex <==
\makeatletter

%%%%%%% ░░ Packages ░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░
	\PassOptionsToPackage{dvipsnames}{xcolor}
	\usepackage{amsmath}
	\usepackage{amssymb}
	\usepackage{amsthm}
	\usepackage[USenglish]{babel}
	\usepackage{comment}
	\usepackage{eqparbox}
	\usepackage{enumitem}
	\usepackage[T1]{fontenc}
	\usepackage{mathtools}
	\usepackage{nicefrac}
	\usepackage{tcolorbox}
	\usepackage{tikz}
		\usetikzlibrary{arrows.meta, calc, decorations.pathreplacing, positioning}
	\usepackage{xcolor}
	\usepackage{hyperref}
	\usepackage[capitalize,nameinlink]{cleveref}




%%%%%%% ░░ Class ░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░
	\newcommand{\keywords}[1]{\par\noindent{\bf Keywords. }#1}
	\newcommand{\amssubj}[1]{\par\noindent{\bf AMS subject classifications. }#1}

	\pdfstringdefDisableCommands{%
		\def\and{, }%
		\def\footnotemark{}%
		\def\funding{}%
		\def\thanks{}%
	}%



%%%%%%% ░░ Settings ░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░
	\frenchspacing
	\hypersetup{%
		breaklinks,
		hypertexnames = true,
		plainpages    = false,
		colorlinks = true,
		urlcolor   = MidnightBlue,
		linkcolor  = MidnightBlue,
		citecolor  = ForestGreen,
	}



%%%%%%% ░░ Lists ░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░
	% automatic widest <https://tex.stackexchange.com/a/547398/21001>
	\SetEnumitemKey{widestL}{
		labelwidth=\eqboxwidth{listlabel@\EnumitemId},
		leftmargin=!,
		format=\mylistlabel,
	}
	\newcommand\mylistlabel[2][l]{\eqmakebox[listlabel@\EnumitemId][#1]{#2}}

	\setlist[itemize,1]{
		wide,
		label=\raisebox{0.3ex}{$\bullet$},
		leftmargin = 0pt,
		labelindent = 0pt,
	}
	\setlist[itemize,2]{
		wide,
		label=\raisebox{0.3ex}{\tiny$\bullet$},
		leftmargin = 0pt,
		labelindent = 0pt,
	}

	% plain list, e.g. for theorem items
	\setlist[enumerate,1]{
		label=\text{\upshape{(\roman*)}},
	}
	\setlist{
		widestL,
		topsep=1ex,
		itemsep=0pt,
	}

	\newlist{enumerateq}{enumerate}{1}
	\setlist[enumerateq]{
		label={(\alph*)},
	}



%%%%%%% ░░ Theorems ░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░

	\theoremstyle{plain}
	\newtheorem{theorem}{Theorem}[section]
	%
	\newtheorem{assumption}[theorem]{Assumption}
	\newtheorem{corollary}[theorem]{Corollary}
		\Crefname{corollary}{Corollary}{Corollaries}
	\newtheorem{definition}[theorem]{Definition}
	\newtheorem{lemma}[theorem]{Lemma}

	\theoremstyle{definition}
	\newtheorem{example}[theorem]{Example}
	\newtheorem{remark}[theorem]{Remark}

	\theoremstyle{plain}
	\newtheorem{fact}[theorem]{Fact}
		\Crefname{fact}{Fact}{Facts}


	% to create theorem-compatible enumerate lists
	\newcommand{\createthmlists}[1]{%
		%
		% list for individual statements
		\newlist{#1enumerate}{enumerate}{1}%
		\setlist[#1enumerate,1]{%
			label = \upshape{(\roman*)},%
			ref = \text{\thetheorem(\roman*)},%
		}%
		\crefalias{#1enumeratei}{#1}%
		%
		% list for inter-dependent (e.g. equivalent) statements
		\newlist{#1enumerateq}{enumerate}{1}%
		\setlist[#1enumerateq,1]{%
			label = \upshape{(\alph*)},%
			ref = \text{\thetheorem(\alph*)},%
		}%
		\crefalias{#1enumerateqi}{#1}%
		\AtBeginEnvironment{#1}{%
			\expandafter\let\expandafter\enumerate\csname #1enumerate\endcsname
			\expandafter\let\expandafter\endenumerate\csname end#1enumerate\endcsname
			\expandafter\let\expandafter\enumerateq\csname #1enumerateq\endcsname
			\expandafter\let\expandafter\endenumerateq\csname end#1enumerateq\endcsname
		}{}{}%
	}%

	\createthmlists{corollary}
	\createthmlists{example}
	\createthmlists{fact}
	\createthmlists{lemma}
	\createthmlists{remark}
	\createthmlists{theorem}


	% add \qedsymbol at the end of Examples and remarks
	\newif\ifnoproof\noprooftrue
	\AfterEndEnvironment{proof}{\noprooffalse}
	\newcommand{\addqedto}[2][]{%
		\AtBeginEnvironment{#2}{%
			\global\noprooftrue
			\ifstrempty{#1}{}{%
				\renewcommand{\qedsymbol}{#1}%
			}%
			\pushQED{\qed}%
		}%
		\AtEndEnvironment{#2}{%
			\ifnoproof\popQED\fi
			\global\noprooftrue
		}%
	}

	\addqedto{example}
	\addqedto{remark}




%%%%%%% ░░ Equations ░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░
	\numberwithin{equation}{section}
	\newcommand{\numberthis}{\addtocounter{equation}{1}\tag{\theequation}}% add number to unnumbered equation/align




%%%%%%% ░░ Math ░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░░
	%% Norms
	\DeclarePairedDelimiter\norm{\lVert}{\rVert}
	\DeclarePairedDelimiter\abs{\lvert}{\rvert}
	\newcommand{\innprod}[2]{\langle#1,#2\rangle}


	%% Symbols
	% mathbb variant
		\DeclareSymbolFont{varmathbb}{U}{txmia}{m}{it}
		\DeclareMathSymbol{\m@thbbch@rN}{\mathord}{varmathbb}{142}
		\DeclareMathSymbol{\m@thbbch@rR}{\mathord}{varmathbb}{146}
		\DeclareMathSymbol{\m@thbbch@rZ}{\mathord}{varmathbb}{154}
	\newcommand{\N}{\m@thbbch@rN}
	\newcommand{\R}{\m@thbbch@rR}
	\newcommand{\Rinf}{\overline{\R}}
	\NewDocumentCommand{\X}{s}{\mathcal{X}\IfBooleanT{#1}{^*}}
	\NewDocumentCommand{\Y}{s}{\mathcal{Y}\IfBooleanT{#1}{^*}}
	\def\Nb_#1{\mathcal{N}_{#1}}

	\NewDocumentCommand{\restr}{e{_}}{%
		\mathop{}\!
		\mathchoice
		{\bigr\rvert_{#1}}
		{\bigr\rvert_{#1}}
		{\rvert_{#1}}
		{\rvert_{#1}}
	}
	\NewDocumentCommand{\Restr}{e{_}}{%
		\mathop{}\!
		\mathchoice
		{\Bigr\rvert_{#1}}
		{\Bigr\rvert_{#1}}
		{\rvert_{#1}}
		{\rvert_{#1}}
	}

	\newcommand{\func}[3]{#1:#2\rightarrow#3}
	\newcommand{\ffunc}[3]{#1:#2\rightrightarrows#3}

	\NewDocumentCommand{\defeq}{s O{=}}{%
		\stackrel{\text{\IfBooleanT{#1}{\clap}{(def)}}}{#2}
	}

	\NewDocumentCommand{\seq}{s m e{_^}}{%
		\IfBooleanF{#1}{\left}(
			#2
		\IfBooleanF{#1}{\right})
		\IfValueTF{#3}{_{#3}}{_{k\in\N}}
		\IfValueT{#4}{^{#4}}
	}
	\NewDocumentCommand{\set}{s m o}{%
		\IfBooleanF{#1}{\left}\{
			#2
			\IfValueT{#3}{\mid#3}
		\IfBooleanF{#1}{\right}\}
	}

	\newcommand{\epicomp}{(\nabla\kernel\mathbin{\triangleright} g)}

	% a- and B-convexity
	\RenewDocumentCommand{\a}{s E{_}{\kernel}}{a$_{#2\IfBooleanT{#1}{^*}}$}%
	\NewDocumentCommand{\A}{s E{_}{\kernel}}{A$_{#2\IfBooleanT{#1}{^*}}$}%
	\NewDocumentCommand{\B}{s E{_}{\kernel}}{B$_{#2\IfBooleanT{#1}{^*}}$}%



%% Operators
	\let\oldnabla\nabla
	\renewcommand{\nabla}{\mathop{}\!\oldnabla}
	\let\oldinf\inf
	\def\inf{\@ifstar{\operatorname*{in\vphantom{p}f}}\oldinf}

	\DeclareMathOperator*{\argmax}{arg\,max}
	\DeclareMathOperator*{\argmin}{arg\,min}
	\def\cball(#1,#2){\operatorname{\overline B}(#1,#2)}
	\DeclareMathOperator{\boundary}{bdry}
	\DeclareMathOperator{\closure}{cl}
	\NewDocumentCommand{\conv}{s}{%
		\IfBooleanTF{#1}%
			{\operatorname{\overline{conv}}}%
			{\operatorname{conv}}%
	}
	\DeclareMathOperator{\dom}{dom}
	\DeclareMathOperator{\epi}{epi}
	\DeclareMathOperator{\graph}{gph}
	\DeclareMathOperator{\indicator}{\delta}
	\DeclareMathOperator{\relint}{ri}
	\DeclareMathOperator{\interior}{int}
	\DeclareMathOperator{\range}{ran}

	% Euclidean prox/env/hull
	\NewDocumentCommand{\Eenv}{E{_}{{\text{\red!missing!subscript!}}}}{%
		\mathop{}\!{\operator@font env}_{#1}\mathopen{}
	}%
	\NewDocumentCommand{\Ehull}{E{_}{{\text{\red!missing!subscript!}}}}{%
		\mathop{}\!{\operator@font hull}_{#1}\mathopen{}
	}%
	\NewDocumentCommand{\Eprox}{E{_}{{\text{\red!missing!subscript!}}}}{%
		\mathop{}\!{\operator@font prox}_{#1}\mathopen{}
	}%

	% Euclidean kernel j
	\DeclareFontFamily{U}{boondoxuprscr}{\skewchar \font =45}
	\DeclareFontShape{U}{boondoxuprscr}{m}{n}{
		<-> BOONDOXUprScr-Regular}{}
	\DeclareFontShape{U}{boondoxuprscr}{b}{n}{
		<-> BOONDOXUprScr-Bold}{}

	\DeclareMathAlphabet{\mathboondoxo}{U}{boondoxuprscr}{m}{n}
	\SetMathAlphabet{\mathboondoxo}{bold}{U}{boondoxuprscr}{b}{n}

	\renewcommand\j{\mathboondoxo{j}}


%% Bregman distance

	\let\oldpartial\partial
	\renewcommand{\partial}{{\red\oldpartial}}
	\let\oldphi\phi
	\renewcommand{\phi}{{\red\oldphi}}

	\NewDocumentCommand{\kernel}{s}{\oldphi\IfBooleanT{#1}{^*}}

	\NewDocumentCommand{\D}{s E{_}{\kernel}}{%
		\operatorname{D}_{%
			#2\IfBooleanT{#1}{^*}%
		}%
	}%

	\NewDocumentCommand{\DD}{s E{_}{\kernel}}{%
		\operatorname{\Delta}_{%
			#2\IfBooleanT{#1}{^*}%
		}%
	}%

	\NewDocumentCommand{\prox}{s E{^_}{{\kernel}{\text{\red!missing!subscript!}}}}{%
		\IfBooleanTF{#1}{%
			\mathop{}\!\overrightarrow{\operator@font prox}
		}{%
			\mathop{}\!\overleftarrow{\operator@font prox}
		}%
		_{#3}^{#2}%
	}%
	\NewDocumentCommand{\env}{s E{^_}{{\kernel}{\lambda}}}{%
		\IfBooleanTF{#1}{%
			\mathop{}\!\overrightarrow{\operator@font env}_{#3}^{#2}\mathopen{}
		}{%
			\mathop{}\!\overleftarrow{\operator@font env}_{#3}^{#2}\mathopen{}
		}%
	}%
	\NewDocumentCommand{\hull}{s E{^_}{{\kernel}{\lambda}}}{%
		\IfBooleanTF{#1}{%
			\mathop{}\!\overrightarrow{\operator@font hull}_{#3}^{#2}\mathopen{}
		}{%
			\mathop{}\!\overleftarrow{\operator@font hull}_{#3}^{#2}\mathopen{}
		}%
	}%

	\NewDocumentCommand{\pb}{s e{_^}}{% prox-boundedness threshold
		\IfBooleanTF{#1}{%
			\vec{\lambda}%
			\IfValueTF{#2}{_{#2}}{_{g}}%
			\IfValueTF{#3}{^{#3}}{^{\kernel}}%
		}{%
			\lambda%
			\IfValueTF{#2}{_{#2}}{_{f}}%
			\IfValueTF{#3}{^{#3}}{^{\kernel}}%
		}%
	}%


%% Subdifferentials
	\NewDocumentCommand{\fsubdiff}{e{^}}{%  Fenchel subdifferential
		\mathop{}\!\oldpartial_{\rm F}%
		\IfValueT{#1}{^{{\red#1}}}%
	}
	\NewDocumentCommand{\lsubdiff}{e{_^}}{% limiting subdifferential
		\mathop{}\!\oldpartial%
		\IfValueT{#1}{_{{\red#1}}}%
		\IfValueT{#2}{^{{\red#2}}}%
	}
	\NewDocumentCommand{\rsubdiff}{e{_^}}{% regular subdifferential
		\mathop{}\!\widehat\oldpartial%
		\IfValueT{#1}{_{{\red#1}}}%
		\IfValueT{#2}{^{{\red#2}}}%
	}


%% Phi-conjugacy
	\let\oldPhi\Phi
	\let\oldPsi\Psi
	\renewcommand{\Phi}{{\red\oldPhi}}
	\renewcommand{\Psi}{{\red\oldPsi}}
	\NewDocumentCommand{\Phikernel}{s}{\IfBooleanTF{#1}{\oldPsi}{\oldPhi}}
	\NewDocumentCommand{\subdiff}{s}{\mathop{}\!\oldpartial_{\IfBooleanTF{#1}{\Phikernel*}{\Phikernel}}}	% Phi-subdifferential
	\NewDocumentCommand{\conj}{sm}{#2{}^{\IfBooleanTF{#1}{\Phikernel*}{\Phikernel}}}						% Phi-conjugate
	\NewDocumentCommand{\biconj}{sm}{#2{}^{\IfBooleanTF{#1}{\Phikernel*\Phikernel}{\Phikernel\Phikernel*}}}	% Phi-biconjugate

\makeatother


==> TeX/Tikz/oscusc_otherattempt.tex <==
\begin{tikzpicture}[
	node distance = 0.25cm and 1cm,
	lwidth/.style = {line width = 0.75pt},
	below*/.style = {below = #1, yshift = -1cm},
% 	Yshift/.style = {yshift = 0.75cm},
% 	Yshift*/.style = {yshift = -0.75cm},
	null/.style = {
		box,
		draw = none,
% 		minimum height = 0.5cm,
% 		minimum width = 1.5cm,
	},
	box/.style = {
		draw,
		inner sep = 5pt,
		rounded corners,
% 		outer sep = 10pt,
		minimum width = 1.5cm,
		minimum height = 0.75cm,
		align = center,
	},
	arrow/.style = {
		lwidth,
		> = {Stealth[length=5pt]},
		shorten > = 1pt,
		shorten < = 1pt,
	},
	arrow*/.style = {
		red,
		arrow,
		dashed,
	},
]

	% Define nodes
	\node[box] (gph)   {graph closed in \(X\times\R^n\)};
	\node[box] (osc)   [right = of gph] {osc};
\new{%
	\node[box] (lb)    [left  = of gph] {lb};
}%

	\node[null] (center) [below* = of gph] {};
	\coordinate (temp) at ($(lb.south east)!0.5!(gph.south west)$);
	\node[box] (usckv) at (temp |- center) {usc k-v};

	\node[box] (usccv) [above = of center] {usc c-v};

	\node[box] (lb2)   [below* = of osc ] {lb};

	\node[box] (uscbv) [below = of center ] {usc b-v};
	\node[box] (usc) [below* = of lb2] {usc};

	% Curly braces
	\draw[
		lwidth,
		decorate,
		decoration = {brace, amplitude = 6pt},
	] (usccv.south east) -- (uscbv.north east) node[midway, right] (usccbv) {};
	\draw[
		lwidth,
		decorate,
		decoration = {brace, amplitude = 6pt},
	] (lb2.north west) -- (osc.south west) node[midway, left] (osclb) {};
	\draw[
		lwidth,
		decorate,
		decoration = {brace, amplitude = 6pt},
	] (usc.north west) -- (lb2.south west) node[midway, left] (usclb) {};
\new{%
	\draw[
		lwidth,
		decorate,
		decoration = {brace, amplitude = 6pt},
	] (gph.south west) -- (lb.south east) node[midway, below] (gphlb) {};
}%

	% Connect with arrow arrows
	\draw[arrow, ->, bend right = 20] (usckv.south east) to (uscbv.west);
	\draw[arrow, ->, bend left = 20] (usckv.north east) to (usccv.west);
	\draw[arrow, <->] (uscbv.east) -- (usclb.west);
	\draw[arrow, ->, out = 0, in = 210] (usccv.east) to ([yshift = 3pt]osc.south west);
	\draw[arrow, ->] (usccbv.east) to[out = 0, in = 210] ([yshift = -1pt]osclb.west);

	\draw[arrow, -> ] ([yshift =  3pt]gph.east) -- ([yshift =  3pt]osc.west);
	\draw[arrow*,<- ] ([yshift = -3pt]gph.east) -- ([yshift = -3pt]osc.west);

	\draw[arrow*,->, out = 180, in = 0] ([yshift = 1pt]osclb.west) to (usckv.east);
\new{%
	\draw[arrow ,<->] (usckv.north) to (gphlb.south);
}%
\end{tikzpicture}

